MaRDMO: Future Gateway to FAIR Mathematical Data

Mathematical research data plays a crucial role across scientific disciplines, yet its documentation and dissemination remain challenging due to the lack of standardized research data management practices. The MaRDMO Plugin addresses these challenges by integrating mathematical models, algorithms, and interdisciplinary workflows into the established framework of the Research Data Management Organiser (RDMO). Built on FAIR principles, MaRDMO enables structured documentation and retrieval of mathematical research data through guided questionnaires. It connects to multiple knowledge graphs, including MathModDB, MathAlgoDB, and the MaRDI Portal. Users can document and search for models, algorithms, and workflows via dynamic selection interfaces that also leverage other sources such as Wikidata. The plugin facilitates the export to the individual MaRDI services, ensuring data quality through automated validation. By embedding mathematical research data management into the widely adopted RDMO platform, MaRDMO represents a significant step toward making mathematical research data more findable, accessible, and reusable.

==> tables/table1.tex <==
\begin{table}[ht]
    \caption{\small bwHPC clusters (entrance level).}
    \centering
    \begin{tabular}{ll}
        \hline
        Cluster                & Location            \\
        \hline\hline
        bwUniCluster           & Karlsruhe           \\
        bwForCluster JUSTUS    & Ulm                 \\
        bwForCluster MLS\&WISO & Heidelberg/Mannheim \\
        bwForCluster NEMO      & Freiburg            \\
        bwForCluster BinAC     & Tübingen            \\
        \hline
    \end{tabular}
    
    \label{tab:table1}
\end{table}

